Some Examples of Family Floer Mirrors

In this article, we give explicit calculations for the family Floer mirrors of some non-compact Calabi-Yau surfaces. We compare it with the mirror construction of Gross-Hacking-Keel for suitably chosen log Calabi-Yau pairs and the rank two cluster varieties of finite type. In particular, the analytifications of the later two give partial compactifications of the family Floer mirrors that we computed.

==> recap_analytic.tex <==
\subsubsection*{Analytic geometry}

Let $\Bbbk$ be a non-archimedean field, i.e. the field is complete with respect to a specified nontrivial non-archimedean absolute value $| \cdot |$. 
It would be the Novikov field $\Lambda$ with valuation $\mbox{val}$ \mandy{yu shen check if need exp or not} in this article. 
Denote $R$ as its \emph{valuation ring}
\[
R  = \{ t \in \Bbbk \mid | t | \leq 1 \}.
\]

For $n \geq 1$, the $n$-variable \emph{Tate algebra} over $\Bbbk$ is
\[
T_n = T_n (\Bbbk) = 
\left\{
\sum a_J X^J \mid |a_J| \rightarrow 0 \text{ as } 
|| J|| \rightarrow \infty
\right\},
\]
where for a multi-index $J = \{ j_1, \dots , j_n \}$, we write $X^J$ to denote $\prod X_i^{j_i}$ and $||J|| = \sum_i j_i$. 
So $T_n ( \Bbbk )$ is the subring of formal power series in $\Bbbk [[ X_1, \dots, X_n ]]$ that converge on $R^n$. 
This $\Bbbk $ algebra is denoted $\Bbbk \langle X_1, \dots, X_n \rangle$. 

Then we say a $\Bbbk$-affinoid algebra is a $\Bbbk$-algebra $A$ admitting an isomorphism $A \cong T_n / I$ as a $\Bbbk$-algebras, for some ideal $I \subseteq T_n$. 
The set of maximal ideals of $A$ is denoted as $\mathrm{MaxSpec} (A)$.

\begin{remark}  \label{rk:domain} \cite{conrad2008several}*{Example 2.2.7}
Note that for $a \in A$, the domains $\mathrm{MaxSpec} (A \langle a \rangle ) = \{ |a| \leq 1 \}$ and $\mathrm{MaxSpec}( A \langle  1/a \rangle ) = \{ |a| \geq 1 \}$. 
%This differs from what we would expect in the toric world where there $\mathrm{Spec} \Bbbk[X_1^{\pm}, \dots, X_n^{\pm}] \cong \mathbb{G}_m^n$. 
\end{remark}

